Scalable communication for high-order stencil computations using CUDA-aware MPI

Modern compute nodes in high-performance computing provide a tremendous level of parallelism and processing power. However, as arithmetic performance has been observed to increase at a faster rate relative to memory and network bandwidths, optimizing data movement has become critical for achieving strong scaling in many communication-heavy applications. This performance gap has been further accentuated with the introduction of graphics processing units, which can provide by multiple factors higher throughput in data-parallel tasks than central processing units. In this work, we explore the computational aspects of iterative stencil loops and implement a generic communication scheme using CUDA-aware MPI, which we use to accelerate magnetohydrodynamics simulations based on high-order finite differences and third-order Runge-Kutta integration. We put particular focus on improving intra-node locality of workloads. Our GPU implementation scales strongly from one to $64$ devices at $50\%$--$87\%$ of the expected efficiency based on a theoretical performance model. Compared with a multi-core CPU solver, our implementation exhibits $20$--$60\times$ speedup and $9$--$12\times$ improved energy efficiency in compute-bound benchmarks on $16$ nodes.

==> tikz/fig-stencil-alternative.tex <==
\tikzset{                                                                        
    iso/.style={kite, draw, kite vertex angles=120, outer sep=0pt}               
    %iso/.style={kite, draw, kite vertex angles=120,  minimum size=1cm, outer sep=0pt}
}                                                                                
                                                                                 
\newcommand{\NN}{3}                                                              
\newcommand{\NNLAST}{2}                                                          
\newcommand{\rot}{0}                                                             
\newcommand{\lineshade}{70}

% params: x, y, z, shade, size                                                   
\newcommand{\xysquare}[5]                                                        
{                                                                                
    {\draw[iso, black!#4, very thin] (#1 + 0, #2 + 0, #3) --                     
                                 (#1 + #5, #2 + 0, #3) --                        
                                 (#1 + #5, #2 + #5, #3) --                       
                                 (#1 + 0, #2 + #5, #3) --                        
                                 (#1 + 0, #2 + 0, #3);}                          
}                                                                                
                                                                                 
\newcommand{\xzsquare}[2]                                                        
{                                                                                
    {\draw[iso, black!20, very thin] (#1 + 0, 0, #2 + 0) --                      
                                 (#1 + 1, 0, #2 + 0) --                          
                                 (#1 + 1, 0, #2 + 1) --                          
                                 (#1 + 0, 0, #2 + 1) --                          
                                 (#1 + 0, 0, #2 + 0);}                           
}                                                                                
                                                                                 
\newcommand{\xzsquareUUSI}[5]                                                    
{                                                                                
    {\draw[iso, black!#4, very thin] (#1 + 0, #3, #2 + 0) --                     
                                 (#1 + #5, #3, #2 + 0) --                        
                                 (#1 + #5, #3, #2 + #5) --                       
                                 (#1 + 0, #3, #2 + #5) --                        
                                 (#1 + 0, #3, #2 + 0);}                          
}                                                                                
                                                                                 
\newcommand{\yzsquare}[5]                                                        
{                                                                                
    {\draw[iso, black!#4, very thin] (#3, #1 + 0, #2 + 0) --                     
                                 (#3, #1 + #5, #2 + 0) --                        
                                 (#3, #1 + #5, #2 + #5) --                       
                                 (#3, #1 + 0, #2 + #5) --                        
                                 (#3, #1 + 0, #2 + 0);}                          
}

    \tdplotsetmaincoords{71.5}{38}{0}
            \begin{tikzpicture}[scale = 1, tdplot_main_coords]%[x={({cos(30)*1cm},{sin(30)*1cm})},y={({cos(150)*1cm},{sin(150)*1cm})},z={(0,1cm)}, scale=2]
            % Helper grid
            \foreach \j in {-\NN, ..., \NNLAST} {
                \foreach \i in {-\NN, ..., \NNLAST} {
                    \xysquare{\i}{\j}{-\NN}{25}{1}
                }
            }
            \xysquare{-\NN}{-\NN}{-\NN}{40}{2*\NN}

            \foreach \j in {-\NN, ..., \NNLAST} {
                \foreach \i in {-\NN, ..., \NNLAST} {
                    \xysquare{\i}{\j}{0}{20}{1}
                }
            }
            %\xysquare{-\NN}{-\NN}{0}{35}{\NN}
            \xysquare{-\NN}{-\NN}{0}{40}{2*\NN}



            \iffalse
            \foreach \j in {-\NN, ..., \NNLAST} {
                \foreach \i in {-\NN, ..., \NNLAST} {
                    \xysquare{\i}{\j}{0}{20}
                }
            }

            \foreach \j in {-\NN, ..., \NNLAST} {
                \foreach \i in {-\NN, ..., \NNLAST} {
                    \xzsquare{\i}{\j}
                }
            }

            \foreach \j in {-\NN, ..., \NNLAST} {
                \foreach \i in {-\NN, ..., \NNLAST} {
                    \yzsquare{\i}{\j}
                }
            }
            \fi

            % Edges
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (\i, 0, 0) -- (\i + 1, 0, 0);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (0, \i, 0) -- (0, \i + 1, 0);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (0, 0, \i) -- (0, 0, \i + 1);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (\i, \i, 0) -- (\i + 1, \i + 1, 0);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (\i, -\i, 0) -- (\i + 1, -\i - 1, 0);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (\i, 0, \i) -- (\i + 1, 0, \i + 1);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (\i, 0, -\i) -- (\i + 1, 0, -\i - 1);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (0, \i, \i) -- (0, \i + 1, \i + 1);
            }
            \foreach \i in {-\NN, ..., \NNLAST} {
                \draw[iso, black!\lineshade] (0, \i, -\i) -- (0, \i + 1, -\i - 1);
            }


            % Nodes
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (\i, 0, 0) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (0, \i, 0) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (0, 0, \i) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (\i, \i, 0) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (\i, -\i, 0) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (\i, 0, \i) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (\i, 0, -\i) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (0, \i, \i) [circle, fill=black!100]{};
            }
            \foreach \i in {-\NN, ..., \NN} {
                \node[iso] at (0, \i, -\i) [circle, fill=black!100]{};
            }

            \foreach \j in {-\NN, ..., \NNLAST} {
                \foreach \i in {-\NN, ..., \NNLAST} {
                    \xysquare{\i}{\j}{\NN}{15}{1}
                }
            }
            %\xysquare{-\NN}{-\NN}{\NN}{30}{\NN}
            \xysquare{-\NN}{-\NN}{\NN}{40}{2*\NN}

            \node[iso] at (0, 0, \NN) [circle, fill=black!100]{};
            \node[iso] at (\NN, 0, \NN) [circle, fill=black!100]{};
            \node[iso] at (-\NN, 0, \NN) [circle, fill=black!100]{};
            \node[iso] at (0, \NN, \NN) [circle, fill=black!100]{};
            \node[iso] at (0, -\NN, \NN) [circle, fill=black!100]{};
            \end{tikzpicture}
